ProteinGPT: Multimodal LLM for Protein Property Prediction and Structure Understanding

Understanding biological processes, drug development, and biotechnological advancements requires a detailed analysis of protein structures and functions, a task that is inherently complex and time-consuming in traditional protein research. To streamline this process, we introduce ProteinGPT, a state-of-the-art multimodal large language model for proteins that enables users to upload protein sequences and/or structures for comprehensive analysis and responsive inquiries. ProteinGPT integrates protein sequence and structure encoders with linear projection layers to ensure precise representation adaptation and leverages a large language model (LLM) to generate accurate, contextually relevant responses. To train ProteinGPT, we constructed a large-scale dataset of 132,092 proteins, each annotated with 20-30 property tags and 5-10 QA pairs per protein, and optimized the instruction-tuning process using GPT-4o. Experiments demonstrate that ProteinGPT effectively generates informative responses to protein-related questions, achieving high performance on both semantic and lexical metrics and significantly outperforming baseline models and general-purpose LLMs in understanding and responding to protein-related queries. Our code and data are available at https://github.com/ProteinGPT/ProteinGPT.

==> contents/deprecate.tex <==

\begin{table*}[htbp]
  \centering
  \caption{ROUGE Metrics for Standard Models: 120 proteins x 28\(\sim\)30 questions/protein = 3508 cases}
  \resizebox{0.5\textwidth}{!}{ % This resizes the table to fit the linewidth
    \begin{tabular}{lrrrr}
    \toprule
    \textbf{Model} & \textbf{ROUGE-1} & \textbf{ROUGE-2} & \textbf{ROUGE-L} & \textbf{ROUGE-LSum} \\
    \midrule
    Llama2 & 0.366 & 0.021 & 0.362 & 0.365 \\
    Llama3 & 0.090 & 0.005 & 0.090 & 0.090 \\
    Vicuna & 0.345 & 0.007 & 0.350 & 0.348 \\
    Mistral & 0.472 & 0.048 & 0.471 & 0.470 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:rouge_standard}%
\end{table*}%

\begin{table*}[htbp]
  \centering
  \caption{ROUGE Metrics for MA-Modified Models: 120 proteins x 28\(\sim\)30 questions/protein = 3508 cases}
  \resizebox{0.5\textwidth}{!}{ % This resizes the table to fit the linewidth
    \begin{tabular}{lrrrr}
    \toprule
    \textbf{Model} & \textbf{ROUGE-1} & \textbf{ROUGE-2} & \textbf{ROUGE-L} & \textbf{ROUGE-LSum} \\
    \midrule
    Llama2-MA & 0.063 & 0.004 & 0.064 & 0.064 \\
    Llama3-MA & 0.090 & 0.005 & 0.090 & 0.090 \\
    Vicuna-MA & 0.345 & 0.007 & 0.350 & 0.348 \\
    Mistral-MA & 0.472 & 0.048 & 0.471 & 0.470 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:rouge_ma}%
\end{table*}%

\begin{table*}[htbp]
  \centering
  \caption{BERT and GPT Metrics for Standard Models: 120 proteins x 28\(\sim\)30 questions/protein = 3508 cases}
  \resizebox{0.55\textwidth}{!}{ % This resizes the table to fit the linewidth
    \begin{tabular}{rlrrr}
    \toprule
    \textbf{Metric} & \textbf{Model} & \textbf{BERT\_Score} & \textbf{PubMedBert} & \textbf{GPT\_Score} \\
    \midrule
    \textbf{Precision} & Llama2 & 0.779 & 0.706 & 0.698 \\
                       & Llama3 & 0.593 & 0.487 & 0.446 \\
                       & Vicuna & 0.730 & 0.626 & 0.605 \\
                       & Mistral & 0.825 & 0.764 & 0.724 \\
    \midrule
    \textbf{Recall} & Llama2 & 0.803 & 0.776 & 0.713 \\
                    & Llama3 & 0.695 & 0.456 & 0.309 \\
                    & Vicuna & 0.788 & 0.751 & 0.661 \\
                    & Mistral & 0.844 & 0.820 & 0.759 \\
    \midrule
    \textbf{F1 Score} & Llama2 & 0.790 & 0.739 & 0.705 \\
                      & Llama3 & 0.638 & 0.470 & 0.363 \\
                      & Vicuna & 0.756 & 0.682 & 0.630 \\
                      & Mistral & 0.834 & 0.790 & 0.740 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:bert_gpt_standard}%
\end{table*}%

\begin{table*}[htbp]
  \centering
  \caption{BERT and GPT Metrics for MA-Modified Models: 120 proteins x 28\(\sim\)30 questions/protein = 3508 cases}
  \resizebox{0.55\textwidth}{!}{ % This resizes the table to fit the linewidth
    \begin{tabular}{rlrrr}
    \toprule
    \textbf{Metric} & \textbf{Model} & \textbf{BERT\_Score} & \textbf{PubMedBert} & \textbf{GPT\_Score} \\
    \midrule
    \textbf{Precision} & Llama2-MA & 0.589 & 0.446 & 0.414 \\
                       & Llama3-MA & 0.593 & 0.487 & 0.446 \\
                       & Vicuna-MA & 0.730 & 0.626 & 0.605 \\
                       & Mistral-MA & 0.825 & 0.764 & 0.724 \\
    \midrule
    \textbf{Recall} & Llama2-MA & 0.679 & 0.477 & 0.308 \\
                    & Llama3-MA & 0.695 & 0.456 & 0.309 \\
                    & Vicuna-MA & 0.788 & 0.751 & 0.661 \\
                    & Mistral-MA & 0.844 & 0.820 & 0.759 \\
    \midrule
    \textbf{F1 Score} & Llama2-MA & 0.628 & 0.459 & 0.351 \\
                      & Llama3-MA & 0.638 & 0.470 & 0.363 \\
                      & Vicuna-MA & 0.756 & 0.682 & 0.630 \\
                      & Mistral-MA & 0.834 & 0.790 & 0.740 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:bert_gpt_ma}%
\end{table*}%










\section{Introduction}

These instructions are for authors submitting papers to ACL 2024 using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} as well as guidelines set forth in the ACL 2024 call for papers.\footnote{\url{https://2024.aclweb.org/calls/main_conference/}} This document contains additional instructions for the \LaTeX{} style files.
The templates include the \LaTeX{} source of this document (\texttt{acl2024.tex}),
the \LaTeX{} style file used to format it (\texttt{acl2024.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.
\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}
\section{Preamble}
\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{ct1965} & \verb|\citep| & \verb|\cite| \\
\citealp{ct1965} & \verb|\citealp| & no equivalent \\
\citet{ct1965} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{ct1965} & \verb|\citeyearpar| & \verb|\shortcite| \\
\citeposs{ct1965} & \verb|\citeposs| & no equivalent \\
\citep[FFT;][]{ct1965} &  \verb|\citep[FFT;][]| & no equivalent\\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}
The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}
To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{ACL2024}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{ACL2024}
\end{verbatim}
\end{quote}
To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)
Please see the \LaTeX{} source of this document for comments on other packages that may be useful.
Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.
By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}



Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).



\subsection{References}

\nocite{Ando2005,augenstein-etal-2016-stance,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}
You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}
Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.





% \begin{table*}[!h]
%   \centering
%   \caption{Semantic Performance with \model and OpenAI GPT models using protein sequence as text input. $S_{\mathrm{BERT}}$, $S_{\mathrm{Pub}}$, and $S_{\mathrm{GPT}}$ stand for BERTScore~\cite{zhangbertscore}, PubMedBERT Score~\cite{pubmedbert}, and GPT-4o Score~\cite{openai2024gpt4}, respectively.}
%     \begin{tabular}{lccccccc}
%     \toprule
%     Metric & Vicuna & Llama-2 & Llama-3 & Mistral & GPT-3.5-turbo & GPT-4-turbo & GPT-4o \\
%     \midrule
%     Precision & 0.730 & 0.739 & 0.779 & 0.821 & 0.641 & 0.578 & 0.596 \\
%     $S_{\mathrm{BERT}}$ & 0.626 & 0.644 & 0.706 & 0.758 & 0.513 & 0.434 & 0.440 \\
%     $S_{\mathrm{Pub}}$ & 0.605 & 0.606 & 0.698 & 0.717 & 0.470 & 0.391 & 0.391 \\
%     \midrule
%     Recall & 0.788 & 0.796 & 0.803 & 0.839 & 0.701 & 0.675 & 0.668 \\
%     $S_{\mathrm{BERT}}$ & 0.751 & 0.773 & 0.776 & 0.816 & 0.667 & 0.406 & 0.580 \\
%     $S_{\mathrm{Pub}}$ & 0.661 & 0.689 & 0.713 & 0.752 & 0.466 & 0.266 & 0.363 \\
%     \midrule
%     F1 & 0.756 & 0.764 & 0.790 & 0.829 & 0.667 & 0.621 & 0.628 \\
%     $S_{\mathrm{BERT}}$ & 0.682 & 0.701 & 0.739 & 0.784 & 0.579 & 0.418 & 0.499 \\
%     $S_{\mathrm{Pub}}$ & 0.630 & 0.644 & 0.705 & 0.733 & 0.467 & 0.316 & 0.376 \\
%     \bottomrule
%     \end{tabular}
%   \label{tab:compare_semantic}%
% \end{table*}%

% \begin{table*}[htbp]
%   \centering
%   \caption{Semantic Performance with \model and OpenAI GPT models using protein sequence as text input. $S_{\mathrm{BERT}}$, $S_{\mathrm{Pub}}$, and $S_{\mathrm{GPT}}$ stand for BERTScore~\cite{zhangbertscore}, PubMedBERT Score~\cite{pubmedbert}, and GPT-4o Score~\cite{openai2024gpt4}, respectively.}
%     \begin{tabular}{llccccccc}
%     \toprule
%     & & Vicuna & Llama-2 & Llama-3 & Mistral & GPT-3.5-turbo & GPT-4-turbo & GPT-4o \\
%     \midrule
%     \multirow{3}{*}{$S_{\mathrm{BERT}}$} 
%         & Precision & 0.730 & 0.739 & 0.779 & 0.821 & 0.641 & 0.578 & 0.596 \\
%         & Recall & 0.788 & 0.796 & 0.803 & 0.839 & 0.701 & 0.675 & 0.668 \\
%         & F1 & 0.756 & 0.764 & 0.790 & 0.829 & 0.667 & 0.621 & 0.628 \\
%     \midrule
%     \multirow{3}{*}{$S_{\mathrm{Pub}}$} 
%         & Precision & 0.626 & 0.644 & 0.706 & 0.758 & 0.513 & 0.434 & 0.440 \\
%         & Recall & 0.751 & 0.773 & 0.776 & 0.816 & 0.667 & 0.406 & 0.580 \\
%         & F1 & 0.682 & 0.701 & 0.739 & 0.784 & 0.579 & 0.418 & 0.499 \\
%     \midrule
%     \multirow{3}{*}{$S_{\mathrm{GPT}}$} 
%         & Precision & 0.605 & 0.606 & 0.698 & 0.717 & 0.470 & 0.391 & 0.391 \\
%         & Recall & 0.661 & 0.689 & 0.713 & 0.752 & 0.466 & 0.266 & 0.363 \\
%         & F1 & 0.630 & 0.644 & 0.705 & 0.733 & 0.467 & 0.316 & 0.376 \\
%     \bottomrule
%     \end{tabular}
%   \label{tab:compare_semantic}%
% \end{table*}%

==> contents/fig/5X1Y.tex <==
\begin{figure}[htbp]
% \vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.9\linewidth]{figures/Demo_inline.pdf}}
\label{fig:5X1Y}
\end{center}

% \caption{\yijia{Placeholder for now, wait for results}}
\caption{ProteinGPT's conversation on Protein 5X1Y.}
% \vskip -0.2in
\end{figure}

